Cooperative Multi-agent Approach for Automated Computer Game Testing

Automated testing of computer games is a challenging problem, especially when lengthy scenarios have to be tested. Automating such a scenario boils down to finding the right sequence of interactions given an abstract description of the scenario. Recent works have shown that an agent-based approach works well for the purpose, e.g. due to agents' reactivity, hence enabling a test agent to immediately react to game events and changing state. Many games nowadays are multi-player. This opens up an interesting possibility to deploy multiple cooperative test agents to test such a game, for example to speed up the execution of multiple testing tasks. This paper offers a cooperative multi-agent testing approach and a study of its performance based on a case study on a 3D game called Lab Recruits.

==> Result.tex <==
The results of testing the LR game using the setups outlined in previous sections are represented and discussed in this section. 

\begin{quote}
{\bf RQ:} {\em Does the multi-agent approach improve test performance?}
\end{quote} 

\subsection{Effect of world size and sharing level}

We run our multi-agent setup on ten levels, variations of $Basic{\text -}Level$ with increasing size. For each level, we deployed two agents. One agent is set to use the task selection heuristic $A_H$, and the other $A_L$. The agents' visibility range is six in this experiment. Fig. \ref{fig.multi-single-time} shows the results. 

The graph shows that the multi-agent setup outperforms the single agent setup. %examine the game in terms of time as the level size increases. 
It takes nearly twice as long for a single agent to finish the $100{\times} 100$ level. On small levels, e.g. $10{\times} 10$, the gain is not much.

Fig. \ref{fig.sharedPoint} shows the points collected after a specific time. Recall that opening a door gives point, so the collected total points correlates with the number of tasks completed. When a total of 70 points is reached, all tasks are completed. A single agent needs seven minutes to get to 35 points (half of the total); two agents can get there in five minutes. In 7 minutes, a multi-agent configuration nearly achieves the full point (65), but a single agent takes more than twice as long.
\MyNOTE{Discuss the proposal 1:10 instead of 5:10. Because then sharper rise in the graph indicates important tasks being completed.
We can then perhaps say that multi can complete all important tasks in 3m, for example.
}



\begin{figure}[h]
\centering
\includegraphics[width=\linewidth,height=5cm,scale=0.5]{single-multi-multishared-time.png}
\caption{\rm\em Comparing the time needed to solve all the given tasks in a single-agent setup with a multi-agent setup. 
The $x$-axis is the level size, e.g. $20{\times}20$.
The $y$-axis is time in second. 
$Multi{\text -}agent{\text -}basic$ uses the $basicSync$ cooperation level; $Multi{\text -}agent{\text -}advance$ uses  $advancedSync$.}
\label{fig.multi-single-time}
\vspace{-3mm}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth,height=5cm,scale=0.5]{collected points.png}
\caption{\rm\em Points collected over time on a level with size $100{\times}100$. Collected points correlate with the number of done tasks.}
\label{fig.sharedPoint}
\vspace{-3mm}
\end{figure}


The produced levels using $basic level$ are studied regarding the effect of the cooperation level. We assess the duration required to complete every task in a multi-agent system with both basic and advanced synchronization levels. Agents with advanced synchronization perform better in general, as seen in the graph \ref{fig.multi-single-time}. 



The graph in Fig. \ref{fig.multi-single-time} shows that agents with advanced synchronization perform better as the level size grows, despite the overhead of having to synchronize more information. When an agent chooses a task whose target object $o$ it has never seen before, the shared navigation information from other agents helps it to find $o$, saving time that is otherwise needed for exploring the world in order to find it. In contrast, basic synchronization does share the locations of target objects, but not the path to them. So in this case the agent will have to search the level to locate $o$. 

\subsubsection{Starting position} 
Using $basic{\text -}level$ of size 100, we generated four distinct versions of this level, with each agent placed in four different locations. Fig. X shows the design of these four locations. The effect of the starting location is shown in  graph. X.


\begin{figure}[h]
\centering
\includegraphics[width=\linewidth,height=5cm,scale=0.5]{starting-location.png}
\caption{\rm\em Different view distance in a basic level with the size 100.}
\label{fig.startingLocation}
\vspace{-3mm}
\end{figure}




\subsubsection{View distance}

To test the efficacy \MyNOTE{efficacy is a wrong word here :)} of the agent's view range, we used $basic{\text -}level$ with the size of $100{\times}100$. The results of running the experiment with various view distances are shown in Fig. \ref{fig.viewDistanceMulti}. It demonstrates that when the view distance increases, test performance improves. When examining the experiment more thoroughly, we can observe that by increasing the view distance, the agent sees more objects/tasks in each step and can choose a task based on how far it is from its position. A larger view distance, however, does not significantly alter performance for a single agent. The reason is that, even though the locations are known, the agent still needs to navigate to each task in order to solve it, and this costs time.
\MyNOTE{But Fig. \ref{fig.viewDistanceMulti} only shows for multi-agent, no?}\Samira{yes}

It should be noted that enlarging the view distance may not be an option provided by the game under test, e.g. to keep the amount of data that the game needs to send over to the agents light weight.

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth,height=5cm,scale=0.5]{viewDistanceMulti.png}
\caption{\rm\em Different view distance in a basic level with the size 100 in multi-agent setup.}
\label{fig.viewDistanceMulti}
\vspace{-3mm}
\end{figure}






\subsubsection{Agents with no task priority}
We set up an experiment to investigate the effectiveness of our strategy without dividing tasks among agents and letting them try a task as soon as they saw it. In this setup, we used $basic-level$ with a size of 100 with different view distance. 


\begin{figure}[h]
\centering
\includegraphics[width=\linewidth,height=5cm,scale=0.5]{viewDistanceWith3Setup.png}
\caption{\em Different view distances in a basic level with the size $100{\times}100$. Comparing the performance in single agent setup with multi-agent setup with $selectTaskH$ and without. $MWithH$ means multi-agent with $selectTaskH$ and $MWithoutH$ is without heuristic.}
\label{fig.viewDistanceWith3Setup}
\vspace{-3mm}
\end{figure}

\subsubsection{3 agents setup}
In all the above experiments, we used two agents to gain insight into how multi-agent approach would perform compared to a single agent. In this experiment, we chose $basic level$ with size 100 and put different numbers of agents to solve all given tasks.

n

\begin{quote}
{\bf RQ:} {\em How well can multi-agent deal with complex logic?}
\end{quote}

\subsection{Effect of Game Logic}

\subsubsection{Distant-connection logic}
To investigate how well a multi-agent setup can deal with the distant-connection logic, a $basic{\text -}level$ of size $30{\times}30$ is used. We randomly place the buttons in different locations. We created five different instances of $basic{\text -}level$ with different numbers of doors with distant buttons/enablers, 
starting from two to ten. We compare a single agent with two different synchronization levels in our multi-agents setup. 

Fig \ref{fig.randomconnection} shows the result. Multi-agents with advanced synchronization can perform better than the other two setups. However, on some levels, the difference is not big. The likely cause is accidental tasks solving. This happens when an agent unintentionally completes a task that is not intended for it. This occurs when the agent interacts with $i'$ that is linked to $d'$ while searching for an enabler to open a door $d$.
The task $T_{d'}$ is then declared as completed, though $T_d$ remains uncompleted. \MyNOTE{This still does not explain why this affects the performance of multi agent...}

The graph shows that when the number of distant enablers increases, the time needed to finish the task is almost the same for all types of approaches \MyNOTE{not quite so. Only on setup 4 and 10.}. Even with advanced sharing, it becomes harder for agents to solve all the tasks. Moreover, the single agent needs more time to finish a level with distant enablers as it has to spend more time to find the right button that opens a door. \MyNOTE{not sure if that last sentence about singel-agent is interesting for your reader... What are you trying to say? }



\begin{figure}[h]
\centering
\includegraphics[width=\linewidth,height=5cm,scale=0.5]{random connection.png}
\caption{\rm\em Effect of having distance connection logic on performance.
}
\label{fig.randomconnection}
\vspace{-3mm}
\end{figure}





\subsubsection{Chained-connection logic} 
Fig. \ref{fig.hiddenButton} shows a level with two 'hidden' buttons, marked by X. This means that to open $dx$, $dy$ must first be opened. If the agents take the tasks in such a way that $dx$ is to be opened by agent $A$ and $dy$ by agent $B$, this presents a challenge. Until $B$ opens $dy$, $dx$ cannot be opened. So, $A$ has to wait, and we lose parallelism. Note that the doors' logic is not known to the agents upfront, so it also not possible for the agents to know upfront what an ideal task distribution is. Three distinct levels are created, each with a unique arrangement of one, two, and three hidden buttons. Our comparison of the time required to complete all tasks is shown in Fig. \ref{fig.hiddenButton}. 

The single-agent setup outperforms the multi-agent setup \MyNOTE{basic or advanced sync btw?}. As previously mentioned, one of the causes is the choices the agents made when selecting the tasks to do. The choices taken may force an agent to wait for another agent in order to access to certain areas, and hence the overall tasks solving becomes longer. Secondly, by attempting random buttons that are actually not connected to the door that guards a target room, the agent may block access to another area. 

Generally, we believe that optimally dealing with chained-connections is hard for a multi agent setup, unless some information about the chained logic is known upfront, so the agents could make a better plan to deal with it.

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth,height=5cm,scale=0.5]{hiddenButton.png}
\caption{\rm\em Hidden button design \MyNOTE{caption should be improved.}
}
\label{fig.hiddenButton}
\vspace{-3mm}
\end{figure}

%\textbf{hidden button: share prolog.}
%We believe that sharing the connection found by each agent would affect the performance of having a hidden button by multi-agent. To examine this hypothesis, in addition to advanced synchronization, we share the list of the connections found by each agent. This would help other agents to access a blocked area if it was accessible before.  how it works if we share the connection as well

\subsubsection{Multi-connection logic}
We consider the $basic{\text -}level$ with size 30, where two enablers are connected to multiple blockers, to investigate the impact of multi-connection on performance. Fig. \ref{X} serves as an illustration.





